Expected Return Causes Outcome-Level Mode Collapse in Reinforcement Learning and How to Fix It with Inverse Probability Scaling

Many reinforcement learning (RL) problems admit multiple terminal solutions of comparable quality, where the goal is not to identify a single optimum but to represent a diverse set of high-quality outcomes. Nevertheless, policies trained by standard expected return maximization routinely collapse onto a small subset of outcomes, a phenomenon commonly attributed to insufficient exploration or weak regularization. We show that this explanation is incomplete: outcome level mode collapse is a structural consequence of the expected-return objective itself. Under idealized learning dynamics, the log-probability ratio between any two outcomes evolves linearly in their reward difference, implying exponential ratio divergence and inevitable collapse independent of the exploration strategy, entropy regularization, or optimization algorithm. We identify the source of this pathology as the probability multiplier inside the expectation and propose a minimal correction: inverse probability scaling, which removes outcome-frequency amplification from the learning signal, fundamentally changes the learning dynamics, and provably yields reward-proportional terminal distributions, preventing collapse in multimodal settings. We instantiate this principle in Group Relative Policy Optimization (GRPO) as a drop-in modification, IPS-GRPO, requiring no auxiliary models or architectural changes. Across different reasoning and molecular generation tasks, IPS-GRPO consistently reduces outcome-level mode collapse while matching or exceeding baseline performance, suggesting that correcting the objective rather than adding exploration heuristics is key to reliable multimodal policy optimization.

==> FIG.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{plots/grid_density_heatmaps.pdf}
  \caption{
  Learned terminal-state distributions on the 2D hyper-grid.
  (a) Target reward-induced distribution $p(x) \propto R(x)$.
  (b) GRPO and (c) FlowRL collapse onto a single high-reward mode despite multiple symmetric optima.
  (d) IPS-GRPO successfully recovers all modes and closely matches the target distribution.
  Reported values denote $\ell_1$ distance between the learned and target distributions.
  }
  \label{fig:grid_density}
\end{figure}



\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Method} & $\boldsymbol{n=2}$ & $\boldsymbol{n=4}$ \\
\midrule
GRPO    & $2.8 \times 10^{-2}$ & $5.2 \times 10^{-4}$ \\
FlowRL & $2.8 \times 10^{-2}$ & $5.2 \times 10^{-4}$ \\
\textbf{IPS-GRPO} & $\mathbf{3.0 \times 10^{-3}}$ & $\mathbf{3.7 \times 10^{-4}}$ \\
\bottomrule
\end{tabular}
\caption{$\ell_1$ distance between the learned terminal-state distribution and the target distribution on the hyper-grid domain. Lower is better.}
\label{tab:grid_l1}
\end{table}

\begin{figure*}[t]
    \centering

    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/hypospace_causal.pdf}
        \caption{Causal inference}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/hypospace_3d.pdf}
        \caption{3D voxel reconstruction}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/hypospace_boolean.pdf}
        \caption{Boolean/DNA interaction}
    \end{subfigure}

    \caption{
    Average number of distinct admissible modes recovered as a function of the number of samples drawn from the trained policy.
    Across all three HypoSpace domains, IPS-GRPO steadily discovers new modes with increased sampling, while GRPO and FlowRL saturate early, indicating outcome-level mode collapse.
    }
    \label{fig:hypospace_combined}
\end{figure*}
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Causal Inference} & \textbf{3D Reconstruction} & \textbf{Boolean/DNA} \\
\midrule
GRPO    & $16.02\% \pm 0.35\%$ & $31.61\% \pm 0.01\%$ & $9.50\% \pm 0.00\%$ \\
FlowRL & $12.82\% \pm 0.05\%$ & $26.85\% \pm 0.37\%$ & $10.74\% \pm 0.00\%$ \\
\textbf{IPS-GRPO} 
& $\mathbf{43.91\% \pm 1.39\%}$ 
& $\mathbf{90.00\% \pm 1.24\%}$ 
& $\mathbf{60.74\% \pm 0.78\%}$ \\
\bottomrule
\end{tabular}
\caption{Final recovery rate (\%) on HypoSpace tasks. Higher is better.}
\label{tab:hypospace_results}
\end{table*}





\begin{table}[t]
\centering
\small
\begin{tabular}{c c c c}
\toprule
\textbf{Threshold} & \textbf{Algorithm} & \textbf{Yield} $\uparrow$ & \textbf{OB100} $\downarrow$ \\
\midrule
\multicolumn{4}{c}{\textbf{SYNTH}} \\
0.80 & REINVENT & $5695 \pm 173$  & $605 \pm 41$ \\
0.80 & IPS-GRPO   & $\mathbf{7371 \pm 212}$ & $\mathbf{554 \pm 34}$ \\
0.85 & REINVENT & $418 \pm 78$ & $2934 \pm 68$ \\
0.85 & IPS-GRPO   & $\mathbf{1580 \pm 58}$ & $\mathbf{1178 \pm 43}$ \\
\midrule
\multicolumn{4}{c}{\textbf{ALL-AMIDE}} \\
0.80 & REINVENT & $1 \pm 1$ & $>5000$ \\
0.80 & IPS-GRPO   & $\mathbf{1478 \pm 102}$ & $\mathbf{773 \pm 51}$ \\
0.85 & REINVENT & $0$ & $>5000$ \\
0.85 & IPS-GRPO   & $\mathbf{20 \pm 12}$ & $>5000$ \\
\bottomrule
\end{tabular}
\caption{Molecular optimization results. Yield denotes the number of unique molecules exceeding the reward threshold; OB100 denotes oracle calls required to find 100 such molecules. The oracle budget for SYNTH is 10,000 and for ALL-AMIDE is 5,000}
\label{tab:drug_results}
\end{table}




\begin{table}[t]
\centering
\small
\begin{tabular}{c c c c}
\toprule
\textbf{Group size \(G\)} & \(\boldsymbol{\epsilon=0.01}\) & \(\boldsymbol{\epsilon=0.1}\) & \(\boldsymbol{\epsilon=0.2}\) \\
\midrule
4  & $17.63 \pm 0.33$ & $17.63 \pm 0.33$ & $17.63 \pm 0.33$ \\
8  & $27.50 \pm 0.67$ & $27.50 \pm 0.67$ & $41.99 \pm 0.80$ \\
16 & $41.02 \pm 0.60$ & $33.05 \pm 0.62$ & $\mathbf{43.91 \pm 1.39}$ \\
32 & $32.13 \pm 0.42$ & $35.27 \pm 1.01$ & $25.62 \pm 1.65$ \\
64 & $36.52 \pm 0.32$ & $39.12 \pm 1.33$ & $42.19 \pm 0.14$ \\
\bottomrule
\end{tabular}
\caption{Recovery rate (\%) on HypoSpace causal inference for different group sizes \(G\) and probability clipping thresholds \(\epsilon\). Higher recovery rate is better.}
\label{tab:ablation_g_eps}
\end{table}





\begin{figure}[t]
    \centering

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/why_density.pdf}
        \caption{Sampling density}
        \label{fig:sampling_density}
    \end{subfigure}

    \vspace{0.5em}

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/why_quiver.pdf}
        \caption{Policy Force Field}
        \label{fig:force_field}
    \end{subfigure}

    \vspace{0.5em}

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/why_mode_frequency.pdf}
        \caption{Mode frequency}
        \label{fig:mode_frequency}
    \end{subfigure}

    % \vspace{0.5em}

    \caption{Caption}
    \label{fig:placeholder}
\end{figure}
